SoK: Measuring Blockchain Decentralization

In the context of blockchain systems, the importance of decentralization is undermined by the lack of a widely accepted methodology to measure it. To address this gap, we set out a systematization effort targeting the decentralization measurement workflow. To facilitate our systematization, we put forth a framework that categorizes all measurement techniques used in previous work based on the resource they target, the methods they use to extract resource allocation, and the functions they apply to produce the final measurements. We complement this framework with an empirical analysis designed to evaluate whether the various pre-processing steps and metrics used in prior work capture the same underlying concept of decentralization. Our analysis brings about a number of novel insights and observations. First, the seemingly innocuous choices performed during data extraction, such as the size of estimation windows or the application of thresholds that affect the resource distribution, have important repercussions when calculating the level of decentralization. Second, exploratory factor analysis suggests that in Proof-of-Work (PoW) blockchains, participation on the consensus layer is not correlated with decentralization, but rather captures a distinct signal, unlike in Proof-of-Stake (PoS) systems, where the different metrics align under a single factor. These findings challenge the long-held assumption within the blockchain community that higher participation drives higher decentralization. Finally, we combine the results of our empirical analysis with first-principles reasoning to derive practical recommendations for researchers that set out to measure blockchain decentralization, and we further systematize the existing literature in line with these recommendations.

==> sections/cons_correlation_tables.tex <==
\begin{table*}[]
   %\centering
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.83 & {\cellcolor{LimeGreen}} 0.80 & {\cellcolor{GreenYellow}} 0.47 & {\cellcolor{pink}} -0.37 & {\cellcolor{yellow}} 0.04 \\
hhi & {\cellcolor{LimeGreen}} 0.83 & {\cellcolor{green}} 1.00 & {\cellcolor{green}} 0.94 & {\cellcolor{yellow}} 0.03 & {\cellcolor{yellow}} 0.16 & {\cellcolor{GreenYellow}} 0.37 \\
tau=0.5 & {\cellcolor{LimeGreen}} 0.80 & {\cellcolor{green}} 0.94 & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} 0.02 & {\cellcolor{yellow}} 0.06 & {\cellcolor{GreenYellow}} 0.39 \\
reward entities & {\cellcolor{GreenYellow}} 0.47 & {\cellcolor{yellow}} 0.03 & {\cellcolor{yellow}} 0.02 & {\cellcolor{green}} 1.00 & {\cellcolor{orange}} -0.66 & {\cellcolor{pink}} -0.46 \\
wallet entities & {\cellcolor{pink}} -0.37 & {\cellcolor{yellow}} 0.16 & {\cellcolor{yellow}} 0.06 & {\cellcolor{orange}} -0.66 & {\cellcolor{green}} 1.00 & {\cellcolor{GreenYellow}} 0.39 \\
 tx volume usd & {\cellcolor{yellow}} 0.04 & {\cellcolor{GreenYellow}} 0.37 & {\cellcolor{GreenYellow}} 0.39 & {\cellcolor{pink}} -0.46 & {\cellcolor{GreenYellow}} 0.39 & {\cellcolor{green}} 1.00 \\
\end{tabular}

   \caption{Bitcoin correlations - Consensus layer}
   \label{tab:btc-cons-correlation}
\end{table*}


\begin{table*}[]
   %\centering
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{green}} 1.00 & {\cellcolor{green}} 0.98 & {\cellcolor{LimeGreen}} 0.89 & {\cellcolor{green}} 0.93 & {\cellcolor{lime}} 0.53 \\
hhi & {\cellcolor{green}} 1.00 & {\cellcolor{green}} 1.00 & {\cellcolor{green}} 0.98 & {\cellcolor{LimeGreen}} 0.88 & {\cellcolor{green}} 0.94 & {\cellcolor{lime}} 0.52 \\
tau=0.5 & {\cellcolor{green}} 0.98 & {\cellcolor{green}} 0.98 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.87 & {\cellcolor{green}} 0.91 & {\cellcolor{lime}} 0.50 \\
reward entities & {\cellcolor{LimeGreen}} 0.89 & {\cellcolor{LimeGreen}} 0.88 & {\cellcolor{LimeGreen}} 0.87 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.89 & {\cellcolor{lime}} 0.70 \\
wallet entities & {\cellcolor{green}} 0.93 & {\cellcolor{green}} 0.94 & {\cellcolor{green}} 0.91 & {\cellcolor{LimeGreen}} 0.89 & {\cellcolor{green}} 1.00 & {\cellcolor{lime}} 0.63 \\
 tx volume usd & {\cellcolor{lime}} 0.53 & {\cellcolor{lime}} 0.52 & {\cellcolor{lime}} 0.50 & {\cellcolor{lime}} 0.70 & {\cellcolor{lime}} 0.63 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   \caption{Cardano correlations - Consensus layer}
   \label{tab:ada-cons-correlation}
\end{table*}

\begin{table*}[]
   %\centering
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.81 & {\cellcolor{GreenYellow}} 0.43 & {\cellcolor{pink}} -0.41 & {\cellcolor{LimeGreen}} 0.74 & {\cellcolor{LimeGreen}} 0.71 \\
hhi & {\cellcolor{LimeGreen}} 0.81 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.73 & {\cellcolor{pink}} -0.46 & {\cellcolor{lime}} 0.68 & {\cellcolor{lime}} 0.61 \\
tau=0.5 & {\cellcolor{GreenYellow}} 0.43 & {\cellcolor{LimeGreen}} 0.73 & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} -0.12 & {\cellcolor{yellow}} 0.28 & {\cellcolor{yellow}} 0.16 \\
reward entities & {\cellcolor{pink}} -0.41 & {\cellcolor{pink}} -0.46 & {\cellcolor{yellow}} -0.12 & {\cellcolor{green}} 1.00 & {\cellcolor{OrangeRed}} -0.72 & {\cellcolor{orange}} -0.60 \\
wallet entities & {\cellcolor{LimeGreen}} 0.74 & {\cellcolor{lime}} 0.68 & {\cellcolor{yellow}} 0.28 & {\cellcolor{OrangeRed}} -0.72 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.83 \\
 tx volume usd & {\cellcolor{LimeGreen}} 0.71 & {\cellcolor{lime}} 0.61 & {\cellcolor{yellow}} 0.16 & {\cellcolor{orange}} -0.60 & {\cellcolor{LimeGreen}} 0.83 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   \caption{Ethereum PoW correlations - Consensus layer}
   \label{tab:eth-pow-cons-correlation}
\end{table*}

\begin{table*}[]
   %\centering
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} 0.30 & {\cellcolor{lime}} 0.67 & {\cellcolor{green}} 0.92 & {\cellcolor{orange}} -0.63 & {\cellcolor{lime}} 0.65 \\
hhi & {\cellcolor{yellow}} 0.30 & {\cellcolor{green}} 1.00 & {\cellcolor{lime}} 0.67 & {\cellcolor{yellow}} 0.15 & {\cellcolor{orange}} -0.69 & {\cellcolor{GreenYellow}} 0.35 \\
tau=0.5 & {\cellcolor{lime}} 0.67 & {\cellcolor{lime}} 0.67 & {\cellcolor{green}} 1.00 & {\cellcolor{lime}} 0.60 & {\cellcolor{orange}} -0.67 & {\cellcolor{lime}} 0.67 \\
reward entities & {\cellcolor{green}} 0.92 & {\cellcolor{yellow}} 0.15 & {\cellcolor{lime}} 0.60 & {\cellcolor{green}} 1.00 & {\cellcolor{pink}} -0.48 & {\cellcolor{lime}} 0.69 \\
wallet entities & {\cellcolor{orange}} -0.63 & {\cellcolor{orange}} -0.69 & {\cellcolor{orange}} -0.67 & {\cellcolor{pink}} -0.48 & {\cellcolor{green}} 1.00 & {\cellcolor{orange}} -0.58 \\
 tx volume usd & {\cellcolor{lime}} 0.65 & {\cellcolor{GreenYellow}} 0.35 & {\cellcolor{lime}} 0.67 & {\cellcolor{lime}} 0.69 & {\cellcolor{orange}} -0.58 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   \caption{Ethereum PoS correlations - Consensus layer}
   \label{tab:eth-pos-cons-correlation}
\end{table*}

\begin{table*}[]
   %\centering
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.89 & {\cellcolor{lime}} 0.67 & {\cellcolor{GreenYellow}} 0.48 & {\cellcolor{OrangeRed}} -0.72 & {\cellcolor{yellow}} 0.25 \\
hhi & {\cellcolor{LimeGreen}} 0.89 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.82 & {\cellcolor{yellow}} 0.23 & {\cellcolor{OrangeRed}} -0.80 & {\cellcolor{GreenYellow}} 0.42 \\
tau=0.5 & {\cellcolor{lime}} 0.67 & {\cellcolor{LimeGreen}} 0.82 & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} 0.20 & {\cellcolor{orange}} -0.59 & {\cellcolor{GreenYellow}} 0.35 \\
reward entities & {\cellcolor{GreenYellow}} 0.48 & {\cellcolor{yellow}} 0.23 & {\cellcolor{yellow}} 0.20 & {\cellcolor{green}} 1.00 & {\cellcolor{pink}} -0.31 & {\cellcolor{yellow}} -0.30 \\
wallet entities & {\cellcolor{OrangeRed}} -0.72 & {\cellcolor{OrangeRed}} -0.80 & {\cellcolor{orange}} -0.59 & {\cellcolor{pink}} -0.31 & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} -0.29 \\
 tx volume usd & {\cellcolor{yellow}} 0.25 & {\cellcolor{GreenYellow}} 0.42 & {\cellcolor{GreenYellow}} 0.35 & {\cellcolor{yellow}} -0.30 & {\cellcolor{yellow}} -0.29 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   \caption{Litecoin correlations - Consensus layer}
   \label{tab:ltc-cons-correlation}
\end{table*}

\begin{table*}[]
   %\centering
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} 0.06 & {\cellcolor{lime}} 0.56 & {\cellcolor{LimeGreen}} 0.73 & {\cellcolor{OrangeRed}} -0.76 & {\cellcolor{yellow}} -0.15 \\
hhi & {\cellcolor{yellow}} 0.06 & {\cellcolor{green}} 1.00 & {\cellcolor{lime}} 0.64 & {\cellcolor{yellow}} -0.08 & {\cellcolor{LimeGreen}} 0.79 & {\cellcolor{GreenYellow}} 0.46 \\
tau=0.5 & {\cellcolor{lime}} 0.56 & {\cellcolor{lime}} 0.64 & {\cellcolor{green}} 1.00 & {\cellcolor{GreenYellow}} 0.43 & {\cellcolor{yellow}} 0.12 & {\cellcolor{yellow}} -0.03 \\
reward entities & {\cellcolor{LimeGreen}} 0.73 & {\cellcolor{yellow}} -0.08 & {\cellcolor{GreenYellow}} 0.43 & {\cellcolor{green}} 1.00 & {\cellcolor{orange}} -0.68 & {\cellcolor{pink}} -0.45 \\
wallet entities & {\cellcolor{OrangeRed}} -0.76 & {\cellcolor{LimeGreen}} 0.79 & {\cellcolor{yellow}} 0.12 & {\cellcolor{orange}} -0.68 & {\cellcolor{green}} 1.00 & {\cellcolor{GreenYellow}} 0.44 \\
 tx volume usd & {\cellcolor{yellow}} -0.15 & {\cellcolor{GreenYellow}} 0.46 & {\cellcolor{yellow}} -0.03 & {\cellcolor{pink}} -0.45 & {\cellcolor{GreenYellow}} 0.44 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   \caption{Tezos correlations - Consensus layer}
   \label{tab:xtz-cons-correlation}
\end{table*}



% \begin{table*}[]
%    %\centering
%    

%    }
%    \caption{ correlations - Consensus layer}
%    \label{tab: correlation}
% \end{table*}


==> sections/factor_analysis.tex <==
\begin{table*}
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}
{ccc@{\hskip 0.4in}cc@{\hskip 0.4in}cc@{\hskip 0.4in}}
\toprule
&\multicolumn{2}{c}{\thead{\textbf{}}} &\multicolumn{2}{c}{\thead {\textbf{Outliers removed}}} & \multicolumn{2}{c}{\thead {\textbf{Outliers transformed}}}\\ 
Rotation: &\multicolumn{2}{c}{\thead{None}} &\multicolumn{2}{c}{\thead {None} }& \multicolumn{2}{c}{\thead {None}}\\
&Factor 1 & Factor 2  &  Factor 1 & Factor 2  & Factor 1 & Factor 2 \\
\midrule
Entropy & \colorbox{CornflowerBlue}{-0.98423618}&  0.17705502 & \colorbox{CornflowerBlue}{-0.98136932} &  0.19233243& \colorbox{CornflowerBlue}{-0.98109212} & 0.18278777\\

Gini &  \colorbox{CornflowerBlue}{0.95733645} &-0.26217184 & \colorbox{CornflowerBlue}{0.95455654}& -0.28033403 & \colorbox{CornflowerBlue} {0.96056228} &-0.2584019\\

HHI & \colorbox{CornflowerBlue}{0.94252816} & 0.26561275 & \colorbox{CornflowerBlue}{0.93879704} & 0.28517658 &\colorbox{CornflowerBlue} {0.96299112}&  0.27551735\\

NC & \colorbox{CornflowerBlue}{-0.89892409}& -0.21671262 & \colorbox{CornflowerBlue}{-0.89600857} &-0.21143375 & \colorbox{CornflowerBlue}{-0.90769024}& -0.227277\\

MPR &  \colorbox{CornflowerBlue}{0.83602248}& \colorbox{gray}{0.49009008}& \colorbox{CornflowerBlue}{0.82626401} & 0.5037361& \colorbox{CornflowerBlue}{0.82796791}  &0.45767294 \\

CL & \colorbox{CornflowerBlue}{-0.91325901} & 0.00385599 & \colorbox{CornflowerBlue}{-0.90746877}&  0.01277117 & \colorbox{CornflowerBlue}{-0.91520368}& -0.00271061\\

\# Parties & -0.29806647  & \colorbox{gray}{0.84493207} & -0.25334706 & \colorbox{gray}{0.855372} & -0.28002327&  \colorbox{gray}{0.84303879}\\

Theil & \colorbox{CornflowerBlue}{0.98423618} & -0.17705502 & \colorbox{CornflowerBlue}{0.98136932} & -0.19233243 & \colorbox{CornflowerBlue}{0.98017611} & -0.19325497\\

\bottomrule
\end{tabular}}
\caption{(Bitcoin) The results from the factor analysis for Bitcoin reveals all metrics clumping together under one latent factor with the number of parties separate. With the untouched data, MPR cross-loads for both these factors.} \label{tab: bitcoinloadings}
\end{table*}

\begin{table*}
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}
{ccc@{\hskip 0.4in}cc@{\hskip 0.4in}cc@{\hskip 0.4in}}
\toprule
&\multicolumn{2}{c}{\thead{\textbf{}}} &\multicolumn{2}{c}{\thead {\textbf{Outliers removed}}} & \multicolumn{2}{c}{\thead {\textbf{Outliers transformed}}}\\ 
Rotation: &\multicolumn{2}{c}{\thead{None}} &\multicolumn{2}{c}{\thead {None} }& \multicolumn{2}{c}{\thead {None}}\\
&Factor 1 & Factor 2  &  Factor 1 & Factor 2  & Factor 1 & Factor 2 \\
\midrule
Entropy & \colorbox{CornflowerBlue}{-0.97920082}  &0.17200375 & \colorbox{CornflowerBlue}{-0.96977711} & 0.2202883& \colorbox{CornflowerBlue}{-0.97825013} & 0.18523895\\

Gini &  \colorbox{CornflowerBlue}{0.94590614} &-0.31483316&\colorbox{CornflowerBlue}{0.94026182}& -0.34340203 &  \colorbox{CornflowerBlue}{0.938896} &  -0.30628728\\

HHI & \colorbox{CornflowerBlue}{0.93315192}&  0.26107064 & \colorbox{CornflowerBlue}{0.94336806}&  0.29787415 &\colorbox{CornflowerBlue}{0.97608791} & 0.22111926\\

NC & \colorbox{CornflowerBlue}{-0.8537327} & -0.22912863 & \colorbox{CornflowerBlue}{-0.78968391} &-0.27905868 & \colorbox{CornflowerBlue}{-0.85079637} &-0.28300487\\

MPR &   \colorbox{CornflowerBlue}{0.82611985}  &\colorbox{gray}{0.48127122} & \colorbox{CornflowerBlue}{0.77142944}  &\colorbox{gray}{0.54295688}& \colorbox{CornflowerBlue} {0.83713493} & \colorbox{gray}{0.44967982}\\

CL & \colorbox{CornflowerBlue}{-0.91509678} &-0.04181053 & \colorbox{CornflowerBlue}{-0.88392786}& -0.05370036 & \colorbox{CornflowerBlue}{-0.91459709} &-0.06453011\\

\# Parties & -0.311715  & \colorbox{gray} {0.77130236} & -0.28408056 & \colorbox{gray}{0.76578403} & -0.31076127 & \colorbox{gray}{0.78608}  \\

Theil & \colorbox{CornflowerBlue}{0.97920082}& -0.17200375 &\colorbox{CornflowerBlue}{0.96977711}& -0.2202883 & \colorbox{CornflowerBlue}{0.97535472} &-0.1835311\\

\bottomrule
\end{tabular}}
\caption{(Bitcoin Cash) Across all three datasets, the EFA for Bitcoin Cash shows us that nearly all metrics clump together under one latent variable, with number of parties in another and MPR cross-loading under both.} \label{tab: bitcoin cash loadings}
\end{table*}

\begin{table*}
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}
{ccc@{\hskip 0.4in}cc@{\hskip 0.4in}cc@{\hskip 0.4in}}
\toprule
&\multicolumn{2}{c}{\thead{\textbf{}}} &\multicolumn{2}{c}{\thead {\textbf{Outliers removed}}} & \multicolumn{2}{c}{\thead {\textbf{Outliers transformed}}}\\ 
Rotation: &\multicolumn{2}{c}{\thead{promax}} &\multicolumn{2}{c}{\thead {oblimin} }& \multicolumn{2}{c}{\thead {promax}}\\
&Factor 1 & Factor 2  &  Factor 1 & Factor 2  & Factor 1 & Factor 2 \\
\midrule
Entropy & \colorbox{CornflowerBlue}{-1.09493446} &  0.33307973 & \colorbox{CornflowerBlue}{-0.99267824}& -0.01491146& \colorbox{CornflowerBlue}{-1.08329338} &  0.30858929\\

Gini &  0.26724435&  \colorbox{gray}{-1.08662085} &\colorbox{CornflowerBlue}{0.98679308} &-0.09823963&  0.16094789 & \colorbox{gray}{-1.01544876}\\
HHI & \colorbox{CornflowerBlue}{0.79910874} &  0.32014239 & \colorbox{CornflowerBlue}{0.48204567}&  \colorbox{gray}{0.64963722}& \colorbox{CornflowerBlue}{0.85970731} & 0.23721743\\

NC & \colorbox{CornflowerBlue}{-0.57655946}&  -0.17259992 &  0.01125596 & \colorbox{gray}{-0.71310342} & \colorbox{CornflowerBlue}{-0.57690664}& -0.19120808\\
MPR &  \colorbox{CornflowerBlue}{0.5718448}  &  \colorbox{gray}{0.3770216}& -0.10199725&  \colorbox{gray}{0.79723326}& \colorbox{CornflowerBlue}{0.5842696}  & 0.32800001\\
CL &\colorbox{CornflowerBlue}{-0.7707356} &  -0.23199704 & \colorbox{CornflowerBlue}{-0.67854123} &-0.28889971 & \colorbox{CornflowerBlue}{-0.7801096}  &-0.23113086\\
\# Parties & 0.0285713 &   \colorbox{gray}{0.95853015} & \colorbox{CornflowerBlue}{0.37599815}& -0.10457202 & -0.04533245  &\colorbox{gray}{0.99659434}\\
Theil & \colorbox{CornflowerBlue}{1.09493446} & -0.3330797 & \colorbox{CornflowerBlue}{0.99267824} & 0.01491146 & \colorbox{CornflowerBlue}{1.07171957}&-0.29057248\\
\bottomrule
\end{tabular}}
\caption{(Ethereum) The EFA for Ethereum looks somewhat different across the three datasets, which is likely due to the large amount of outliers. However, across the three, we can see that entropy, HHI, centralization level, and Theil clump together, while Gini, MPR and number of parties tend to deviate.} \label{tab: ethereumloadings}
\end{table*}

\begin{table*}
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}
{ccc@{\hskip 0.4in}c@{\hskip 0.4in}cc@{\hskip 0.4in}}
\toprule
&\multicolumn{2}{c}{\thead{\textbf{}}}& \textbf{Outliers removed} & \multicolumn{2}{c}{\thead {\textbf{Outliers transformed}}}\\ 
Rotation: &\multicolumn{2}{c}{\thead{promax}} &None& \multicolumn{2}{c}{\thead {promax}}\\
&Factor 1 & Factor 2  &  Factor 1 & Factor 1 & Factor 2 \\
\midrule
Entropy & \colorbox{CornflowerBlue}{-0.80476166} & 0.32566241 & \colorbox{CornflowerBlue}{-0.96734191}& \colorbox{CornflowerBlue}{-0.36809505} & \colorbox{gray}{-0.73767047}\\
Gini &  0.09072413& \colorbox{gray}{-0.92691666}&\colorbox{CornflowerBlue}{0.99218079}&  -0.16737461  &\colorbox{gray}{0.74079928}\\
HHI &  \colorbox{CornflowerBlue}{1.01851246} & 0.05242594&  \colorbox{CornflowerBlue}{0.98985561}& \colorbox{CornflowerBlue}{0.89186714}  &0.16396886\\
NC &  \colorbox{CornflowerBlue}{-0.87277773} &-0.14860334 &\colorbox{CornflowerBlue}{-0.80291083} & \colorbox{CornflowerBlue}{-0.9224675}  & 0.09533865\\
MPR  &  \colorbox{CornflowerBlue}{0.9009198}  & 0.1340387&  \colorbox{CornflowerBlue}{0.8454747}& \colorbox{CornflowerBlue}{0.90589869} &-0.03322098\\
CL  &  \colorbox{CornflowerBlue}{-0.88873678} &-0.07937703 &\colorbox{CornflowerBlue}{-0.8546629} & \colorbox{CornflowerBlue}{-0.79515761} &-0.09972536\\
\# Parties  &  0.21137561  &\colorbox{gray}{1.00560392}& \colorbox{CornflowerBlue}{-0.41042189} & 0.19080213& \colorbox{gray}{-0.76706906}\\
Theil & \colorbox{CornflowerBlue}{0.80476167}& -0.32566241 & \colorbox{CornflowerBlue}{0.96734191} & \colorbox{CornflowerBlue}{0.39226674} & \colorbox{gray}{0.70980843}\\
\bottomrule
\end{tabular}}
\caption{(Litecoin) The EFA for Litecoin revealed one latent variable for all metrics when the outliers were removed, however for both the untouched data and the transformed data (leaving the same number of outliers as there were initially), we Gini and number of parties fall under one latent variable, and all others under another (with entropy and Theil cross-loading in the transformed dataset).} \label{tab: litecoinloadings}
\end{table*}

\begin{table*}
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}
{cc@{\hskip 0.4in}cc@{\hskip 0.4in}cc@{\hskip 0.4in}}
\toprule
&\textbf{}&\multicolumn{2}{c}{\thead {\textbf{Outliers removed}}} & \multicolumn{2}{c}{\thead {\textbf{Outliers transformed}}}\\ 

Rotation: &None&\multicolumn{2}{c}{\thead {varimax} }& \multicolumn{2}{c}{\thead {promax}}\\

&Factor 1 & Factor 1 & Factor 2  & Factor 1 & Factor 2 \\
\midrule

Entropy &\colorbox{CornflowerBlue}{-0.99984847} & \colorbox{CornflowerBlue}{0.71183795} &\colorbox{gray}{-0.70066023}& \colorbox{CornflowerBlue}{-0.8825849}  & 0.16494949\\
Gini  &\colorbox{CornflowerBlue}{0.86877017} &\colorbox{CornflowerBlue}{-0.94026861}& -0.27016348 &  -0.12606757&\colorbox{gray}{-0.96502346}\\
HHI &  \colorbox{CornflowerBlue}{0.9067864}  & -0.063951 &   \colorbox{gray}{0.99453432} &\colorbox{CornflowerBlue}{1.07048998} & 0.13990021\\
NC  & \colorbox{CornflowerBlue}{-0.7737484}  & \colorbox{CornflowerBlue}{0.77198586}& \colorbox{gray}{-0.51827913} & -0.21324797  &\colorbox{gray}{0.76672335}\\
MPR &\colorbox{CornflowerBlue}{0.80934234} & 0.1077014  & \colorbox{gray}{0.9895938}&   \colorbox{CornflowerBlue}{1.01047535} & 0.1422518\\
CL &\colorbox{CornflowerBlue}{-0.80377467}  & \colorbox{CornflowerBlue}{0.98180999}& -0.02682992 & 0.16081747&  \colorbox{gray}{1.1036552}\\
\# Parties  & \colorbox{CornflowerBlue}{-0.93974586} &\colorbox{CornflowerBlue} {0.65836947} &-0.12724294 & \colorbox{CornflowerBlue}{-0.74204298} & 0.22389502\\
Theil & \colorbox{CornflowerBlue}{0.99984847} &\colorbox{CornflowerBlue}{-0.71183795} & \colorbox{gray}{0.70066023} & 0.26826599 &\colorbox{gray}{-0.65472846}\\
\bottomrule
\end{tabular}}
\caption{(Tezos) Data transformation for Tezos left nearly all outliers remaining in the dataset. Across all three analyses, we can see that entropy and number of parties grouped together, with NC and Theil grouping together. Tezo's dataset is not as clear as with other ledgers. \mary{why?}} \label{tab: tezosloadings}
\end{table*}


==> sections/results.tex <==
\subsubsection{Spotlight: Relationship between Participation and Decentralization.}\label{sec:empirical-results}

We have identified the most appropriate metrics to quantify participation and decentralization, so we now turn our attention to the relationship between the two. 
\dimitris{we could repeat here the choices to make reading this section easier}
For each layer and each blockchain in question, we conduct exploratory factor analysis. In each dataset, we use the chosen participation metrics (number of block-producing entities, number of token-holding entities, USD trading volume) and decentralization metrics (Gini coefficient, Herfindahl-Hirschman index, Nakamoto coefficient). The results, showing the number of factors for each ledger and how the different metrics load onto them, can be seen in Figure~\ref{fig:cns-EFA-all} (for consensus) and Figure~\ref{fig:tkn-EFA-all} (for tokenomics).

We also calculate the Spearman rank correlations to confirm the findings and  explore pairwise relationships in a more intuitive way.
We follow established guidelines \cite{mukaka2012guide} to characterize the strength of the correlation coefficient as negligible, low, moderate, high, or very high. %, and we color the cells of Tables \ref{tab:consensus-correlations-all} - \ref{tab:tokenomics-correlations-all} accordingly (with green hues representing positive correlation, red hues negative correlation, and yellow negligible correlation).


%\input{sections/consensus_correlation_table_everything}

\paragraph*{Consensus}


The factor analysis reveals a straightforward story for some ledgers and more nuanced for others. In Bitcoin and Ethereum PoW, we identify two factors, where all decentralization metrics load on one and all participation metrics on the other (with the exception of the Gini coefficient, which we discuss later). This suggests, as we suspected, that decentralization and participation capture different latent factors when describing Bitcoin and Ethereum PoW. 

The story becomes more nuanced for Litecoin and Tezos, where we have more crossover between the participation and decentralization metrics, which makes it difficult to interpret what the latent factors represent. In Litecoin there is only one cross-loading (a variable that is significantly correlated to both latent variables) which is the Gini coefficient. Interestingly, it also cross-loads for Tezos, Bitcoin, and Ethereum PoW. This may indicate that the Gini coefficient, specifically, captures some aspects of a participation metric, perhaps because of its tail sensitivity. 

For Cardano and Ethereum PoS, all metrics (participation and decentralization) load onto a single factor. This suggests that there is a closer relationship between participation and decentralization in these ledgers. Ethereum PoS has much less data than that of Ethereum PoW (13 months versus 57 months), which may explain the difference between the number of these factors. We have seen previously (in Table \ref{fig:EFA-consensus}) that Cardano has noticeably higher values of correlation than other ledgers, which may explain why it only yields one factor. 


%Table \ref{tab:consensus-correlations-all} presents the Spearman correlations between the three decentralization metrics, calculated on the distributions of blocks across entities, and the three participation proxies.

Turning to pairwise correlations, Table~\ref{tab:consensus-correlations-all} confirms there is no consistent correlation, neither in strength nor direction, between decentralization and participation across ledgers.
The relevant values range from $-0.80$ (high negative correlation) to $0.94$ (very high positive correlation), depending on the metric and system in question.

%Let us discuss each participation type in more detail.

One would expect reward entities and Nakamoto Coefficient to be closely related given the former is designed to capture participation in the consensus layer and the latter is designed to capture the security of the consensus layer.
Similarly, HHI is designed to capture concentration in economic production, which easily translates to block production at the consensus layer.
It is therefore surprising that NC and HHI are not correlated to the number of entities that participate by contributing blocks in the majority of systems. 
In fact, the Gini coefficient has the strongest positive correlation with reward entities, with coefficients ranging from $0.47$ to $0.92$, excluding Ethereum PoW that exhibits only negative correlations between decentralization and reward entities. 
Recalling that Gini captures a notion of fairness and NC a notion of security, it appears that participation in the consensus layer is only correlated with fairness, and not security.

The other two participation metrics are less relevant to the consensus layer, and they also display no clear relationship to decentralization metrics at the consensus layer.
Wallet entities participation exhibited negative correlation with consensus decentralization (Ethereum PoS, Litecoin), others mostly positive (Cardano, Ethereum PoW), and others mixed or negligible (Bitcoin, Tezos).
In the case of exchange trading volume, there appears to be little to no relationship to the decentralization on the consensus layer for all systems.

% PARTICIPATION VS DECENTRALISATION EFA TOKENOMICS
% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{figures/tokenomics_all_factor_loadings.eps}
%     \caption{Factor analysis results for participation and decentralization on the tokenomics layer.}
%     \label{fig:tkn-EFA-all}
% \end{figure*}

\paragraph*{Tokenomics}

%\input{sections/tokenomics_correlation_table_everything}
Next we move onto the tokenomics layer. Figure~\ref{fig:tkn-EFA-all} shows the exploratory factor analysis, which revealed two underlying factors for all ledgers. Although promising that we see two latent variables, participation and decentralization metrics, interestingly, do not load together in a consistent way. For example, HHI and Gini loaded onto the same factor for Cardano and Tezos, onto different factors for Ethereum PoW and Bitcoin, and weakly loaded for the others.
A similar ``it depends on the blockchain'' story holds for the Nakamoto coefficient/HHI, and Gini/Nakamoto coefficient.

At the consensus layer, we saw that the Gini coefficient consistently clustered with both participation and decentralization metrics. For the tokenomics layer, we see that it cross-loads (again) for Ethereum PoS and Tezos. However, for other ledgers, the Gini coefficient does not consistently cluster with either specific decentralization or participation metrics. In short, the story we understood at the consensus layer, no longer seems to hold when we look at token ownership. 

This inconsistency may, once again, be due to the difference in data between ledgers. Bitcoin's data spans nearly 13 years, while Ethereum PoS is only 1. Acknowledging the lack of a clear pattern, Table~\ref{tab:tokenomics-correlations-all} % (in the Appendix) 
supplements the results with the Spearman correlations between the decentralization metrics, calculated on the distributions of tokens across token holders, and the different types of participation.
Again, the results paint a more nuanced picture, making it harder to find common patterns across ledgers.
A high-level observation is that the vast majority of the relevant coefficients (bottom left or top right part of each table) across systems  are negative or close to zero, implying that there is no positive correlation between participation and decentralization on the tokenomics layer.

When it comes to reward entities, there are some positive correlations to decentralization, but most of them are weak. Wallet entities are by and large inverse correlated to the different decentralization metrics, with only a couple of exceptions. Trading volume follows a similar pattern, demonstrating negative or negligible correlation in most cases.
On average, the strongest negative correlation is observed between HHI and wallet entities, while the strongest positive correlation is between the Nakamoto coefficient % ($\tau=0.5$) 
and reward entities.

Similarly to the consensus layer, our findings indicate that enhancing participation in different ways does not necessarily lead to better decentralization at the tokenomics layer.


%A possible reason for this is that in the case of tokenomics the number of entities is one or two orders of magnitude larger than in consensus (thousands or millions instead of tens or hundreds) and the distributions of tokens to entities are very heavy-tailed.
%Since the Gini coefficient tends to punish long tails, it is conceivable that a growing 



==> sections/tkn_correlation_tables.tex <==
\begin{table*}[]
   %\centering
   \adjustbox{max width=\textwidth}{
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} -0.19 & {\cellcolor{lime}} 0.65 & {\cellcolor{yellow}} -0.15 & {\cellcolor{yellow}} 0.25 & {\cellcolor{pink}} -0.34 \\
hhi & {\cellcolor{yellow}} -0.19 & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} -0.08 & {\cellcolor{lime}} 0.62 & {\cellcolor{OrangeRed}} -0.82 & {\cellcolor{yellow}} -0.23 \\
tau=0.5 & {\cellcolor{lime}} 0.65 & {\cellcolor{yellow}} -0.08 & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} 0.09 & {\cellcolor{yellow}} 0.10 & {\cellcolor{orange}} -0.58 \\
reward entities & {\cellcolor{yellow}} -0.15 & {\cellcolor{lime}} 0.62 & {\cellcolor{yellow}} 0.09 & {\cellcolor{green}} 1.00 & {\cellcolor{orange}} -0.66 & {\cellcolor{pink}} -0.46 \\
wallet entities & {\cellcolor{yellow}} 0.25 & {\cellcolor{OrangeRed}} -0.82 & {\cellcolor{yellow}} 0.10 & {\cellcolor{orange}} -0.66 & {\cellcolor{green}} 1.00 & {\cellcolor{GreenYellow}} 0.39 \\
 tx volume usd & {\cellcolor{pink}} -0.34 & {\cellcolor{yellow}} -0.23 & {\cellcolor{orange}} -0.58 & {\cellcolor{pink}} -0.46 & {\cellcolor{GreenYellow}} 0.39 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   }
   \caption{Bitcoin correlations - Tokenomics layer}
   \label{tab:btc-tkn-correlation}
\end{table*}

% Cardano
\begin{table*}[]
   %\centering
   \adjustbox{max width=\textwidth}{
   \begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.75 & {\cellcolor{orange}} -0.55 & {\cellcolor{orange}} -0.66 & {\cellcolor{OrangeRed}} -0.85 & {\cellcolor{pink}} -0.31 \\
hhi & {\cellcolor{LimeGreen}} 0.75 & {\cellcolor{green}} 1.00 & {\cellcolor{orange}} -0.67 & {\cellcolor{OrangeRed}} -0.86 & {\cellcolor{OrangeRed}} -0.88 & {\cellcolor{orange}} -0.53 \\
tau=0.5 & {\cellcolor{orange}} -0.55 & {\cellcolor{orange}} -0.67 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.77 & {\cellcolor{LimeGreen}} 0.82 & {\cellcolor{lime}} 0.61 \\
reward entities & {\cellcolor{orange}} -0.66 & {\cellcolor{OrangeRed}} -0.86 & {\cellcolor{LimeGreen}} 0.77 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.89 & {\cellcolor{LimeGreen}} 0.76 \\
wallet entities & {\cellcolor{OrangeRed}} -0.85 & {\cellcolor{OrangeRed}} -0.88 & {\cellcolor{LimeGreen}} 0.82 & {\cellcolor{LimeGreen}} 0.89 & {\cellcolor{green}} 1.00 & {\cellcolor{lime}} 0.63 \\
 tx volume usd & {\cellcolor{pink}} -0.31 & {\cellcolor{orange}} -0.53 & {\cellcolor{lime}} 0.61 & {\cellcolor{LimeGreen}} 0.76 & {\cellcolor{lime}} 0.63 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   }
   \caption{Cardano correlations - Tokenomics layer}
   \label{tab:ada-tkn-correlation}
\end{table*}

% Ethereum PoW
\begin{table*}[]
   %\centering
   \adjustbox{max width=\textwidth}{
   \begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} -0.08 & {\cellcolor{yellow}} -0.06 & {\cellcolor{yellow}} -0.30 & {\cellcolor{yellow}} 0.08 & {\cellcolor{yellow}} -0.08 \\
hhi & {\cellcolor{yellow}} -0.08 & {\cellcolor{green}} 1.00 & {\cellcolor{green}} 0.96 & {\cellcolor{LimeGreen}} 0.74 & {\cellcolor{red}} -0.98 & {\cellcolor{OrangeRed}} -0.80 \\
tau=0.5 & {\cellcolor{yellow}} -0.06 & {\cellcolor{green}} 0.96 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.75 & {\cellcolor{red}} -0.95 & {\cellcolor{OrangeRed}} -0.79 \\
reward entities & {\cellcolor{yellow}} -0.30 & {\cellcolor{LimeGreen}} 0.74 & {\cellcolor{LimeGreen}} 0.75 & {\cellcolor{green}} 1.00 & {\cellcolor{OrangeRed}} -0.72 & {\cellcolor{orange}} -0.60 \\
wallet entities & {\cellcolor{yellow}} 0.08 & {\cellcolor{red}} -0.98 & {\cellcolor{red}} -0.95 & {\cellcolor{OrangeRed}} -0.72 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.83 \\
 tx volume usd & {\cellcolor{yellow}} -0.08 & {\cellcolor{OrangeRed}} -0.80 & {\cellcolor{OrangeRed}} -0.79 & {\cellcolor{orange}} -0.60 & {\cellcolor{LimeGreen}} 0.83 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   }
   \caption{Ethereum PoW correlations - Tokenomics layer}
   \label{tab:eth-pow-tkn-correlation}
\end{table*}

% Ethereum PoS
\begin{table*}[]
   %\centering
   \adjustbox{max width=\textwidth}{
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{green}} 0.96 & {\cellcolor{lime}} 0.64 & {\cellcolor{GreenYellow}} 0.41 & {\cellcolor{red}} -0.96 & {\cellcolor{lime}} 0.51 \\
hhi & {\cellcolor{green}} 0.96 & {\cellcolor{green}} 1.00 & {\cellcolor{lime}} 0.55 & {\cellcolor{GreenYellow}} 0.48 & {\cellcolor{red}} -1.00 & {\cellcolor{lime}} 0.58 \\
tau=0.5 & {\cellcolor{lime}} 0.64 & {\cellcolor{lime}} 0.55 & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} 0.05 & {\cellcolor{orange}} -0.55 & {\cellcolor{yellow}} 0.08 \\
reward entities & {\cellcolor{GreenYellow}} 0.41 & {\cellcolor{GreenYellow}} 0.48 & {\cellcolor{yellow}} 0.05 & {\cellcolor{green}} 1.00 & {\cellcolor{pink}} -0.48 & {\cellcolor{lime}} 0.69 \\
wallet entities & {\cellcolor{red}} -0.96 & {\cellcolor{red}} -1.00 & {\cellcolor{orange}} -0.55 & {\cellcolor{pink}} -0.48 & {\cellcolor{green}} 1.00 & {\cellcolor{orange}} -0.58 \\
 tx volume usd & {\cellcolor{lime}} 0.51 & {\cellcolor{lime}} 0.58 & {\cellcolor{yellow}} 0.08 & {\cellcolor{lime}} 0.69 & {\cellcolor{orange}} -0.58 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   }
   \caption{Ethereum PoS correlations - Tokenomics layer}
   \label{tab:eth-pos-tkn-correlation}
\end{table*}

% Litecoin
\begin{table*}[]
   %\centering
   \adjustbox{max width=\textwidth}{
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.71 & {\cellcolor{lime}} 0.61 & {\cellcolor{GreenYellow}} 0.39 & {\cellcolor{red}} -0.97 & {\cellcolor{GreenYellow}} 0.35 \\
hhi & {\cellcolor{LimeGreen}} 0.71 & {\cellcolor{green}} 1.00 & {\cellcolor{LimeGreen}} 0.81 & {\cellcolor{GreenYellow}} 0.36 & {\cellcolor{orange}} -0.61 & {\cellcolor{GreenYellow}} 0.31 \\
tau=0.5 & {\cellcolor{lime}} 0.61 & {\cellcolor{LimeGreen}} 0.81 & {\cellcolor{green}} 1.00 & {\cellcolor{GreenYellow}} 0.41 & {\cellcolor{pink}} -0.46 & {\cellcolor{yellow}} 0.01 \\
reward entities & {\cellcolor{GreenYellow}} 0.39 & {\cellcolor{GreenYellow}} 0.36 & {\cellcolor{GreenYellow}} 0.41 & {\cellcolor{green}} 1.00 & {\cellcolor{pink}} -0.39 & {\cellcolor{yellow}} -0.15 \\
wallet entities & {\cellcolor{red}} -0.97 & {\cellcolor{orange}} -0.61 & {\cellcolor{pink}} -0.46 & {\cellcolor{pink}} -0.39 & {\cellcolor{green}} 1.00 & {\cellcolor{pink}} -0.37 \\
 tx volume usd & {\cellcolor{GreenYellow}} 0.35 & {\cellcolor{GreenYellow}} 0.31 & {\cellcolor{yellow}} 0.01 & {\cellcolor{yellow}} -0.15 & {\cellcolor{pink}} -0.37 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   }
   \caption{Litecoin correlations - Tokenomics layer}
   \label{tab:ltc-tkn-correlation}
\end{table*}


% Tezos
\begin{table*}[]
   %\centering
   \adjustbox{max width=\textwidth}{
\begin{tabular}{lrrrrrr}
{} & {gini} & {hhi} & {tau=0.5} & {reward entities} & {wallet entities} & { tx volume usd} \\
gini & {\cellcolor{green}} 1.00 & {\cellcolor{pink}} -0.50 & {\cellcolor{yellow}} -0.28 & {\cellcolor{lime}} 0.64 & {\cellcolor{orange}} -0.66 & {\cellcolor{orange}} -0.56 \\
hhi & {\cellcolor{pink}} -0.50 & {\cellcolor{green}} 1.00 & {\cellcolor{green}} 0.95 & {\cellcolor{pink}} -0.31 & {\cellcolor{LimeGreen}} 0.72 & {\cellcolor{yellow}} -0.20 \\
tau=0.5 & {\cellcolor{yellow}} -0.28 & {\cellcolor{green}} 0.95 & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} -0.17 & {\cellcolor{lime}} 0.61 & {\cellcolor{pink}} -0.37 \\
reward entities & {\cellcolor{lime}} 0.64 & {\cellcolor{pink}} -0.31 & {\cellcolor{yellow}} -0.17 & {\cellcolor{green}} 1.00 & {\cellcolor{OrangeRed}} -0.83 & {\cellcolor{yellow}} -0.28 \\
wallet entities & {\cellcolor{orange}} -0.66 & {\cellcolor{LimeGreen}} 0.72 & {\cellcolor{lime}} 0.61 & {\cellcolor{OrangeRed}} -0.83 & {\cellcolor{green}} 1.00 & {\cellcolor{yellow}} 0.13 \\
 tx volume usd & {\cellcolor{orange}} -0.56 & {\cellcolor{yellow}} -0.20 & {\cellcolor{pink}} -0.37 & {\cellcolor{yellow}} -0.28 & {\cellcolor{yellow}} 0.13 & {\cellcolor{green}} 1.00 \\
\end{tabular}
   }
   \caption{Tezos correlations - Tokenomics layer}
   \label{tab:xtz-tkn-correlation}
\end{table*}



%%%%%%%%%%%%%%%%



